Combating Misinformation in Bangladesh: Roles and Responsibilities as Perceived by Journalists, Fact-checkers, and Users

There has been a growing interest within CSCW community in understanding the characteristics of misinformation propagated through computational media, and the devising techniques to address the associated challenges. However, most work in this area has been concentrated on the cases in the western world leaving a major portion of this problem unaddressed that is situated in the Global South. This paper aims to broaden the scope of this discourse by focusing on this problem in the context of Bangladesh, a country in the Global South. The spread of misinformation on Facebook in Bangladesh, a country with a population over 163 million, has resulted in chaos, hate attacks, and killings. By interviewing journalists, fact-checkers, in addition to surveying the general public, we analyzed the current state of verifying misinformation in Bangladesh. Our findings show that most people in the `news audience' want the news media to verify the authenticity of online information that they see online. However, the newspaper journalists say that fact-checking online information is not a part of their job, and it is also beyond their capacity given the amount of information being published online everyday. We further find that the voluntary fact-checkers in Bangladesh are not equipped with sufficient infrastructural support to fill in this gap. We show how our findings are connected to some of the core concerns of CSCW community around social media, collaboration, infrastructural politics, and information inequality. From our analysis, we also suggest several pathways to increase the impact of fact-checking efforts through collaboration, technology design, and infrastructure development.

==> limitation.tex <==
% \section{Limitations and Conclusion}


% \textbf{}

==> notes.tex <==
\section{Notes}
\label{notes}

\noindent
\textbf{Why study Bangladesh?}: Online misinformation has been a serious problem in Bangladesh in recent years like in many other countries. However, due to various reasons such as lack of resource, low media literacy, lack of access to information, lack of freedom of press among many other reasons, made it difficult to combat the spread of online misinformation. There is a gap in existing body of research on this domain about how misinformation is being combated within these limitations. This study aims to close that gap by studying the combat of misinformation in Bangladesh.

\noindent
\textbf{Why study Bangladesh?}:

